Model-Independent Global Search for New High-pT Physics at CDF

Data collected in Run II of the Fermilab Tevatron are searched for indications of new electroweak scale physics. Rather than focusing on particular new physics scenarios, CDF data are analyzed for discrepancies with respect to the standard model prediction. A model-independent approach (Vista) considers the gross features of the data, and is sensitive to new large cross section physics. A quasi-model-independent approach (Sleuth) searches for a significant excess of events with large summed transverse momentum, and is particularly sensitive to new electroweak scale physics that appears predominantly in one final state. This global search for new physics in over three hundred exclusive final states in 927 pb^-1 of ppbar collisions at sqrt(s)=1.96 TeV reveals no such significant indication of physics beyond the standard model.

==> twiddleScriptP.tex <==
$
\twiddleScriptP = 0.46
$.

